Multi-Source to Multi-Target Decentralized Federated Domain Adaptation

Heterogeneity across devices in federated learning (FL) typically refers to statistical (e.g., non-i.i.d. data distributions) and resource (e.g., communication bandwidth) dimensions. In this paper, we focus on another important dimension that has received less attention: varying quantities/distributions of labeled and unlabeled data across devices. In order to leverage all data, we develop a decentralized federated domain adaptation methodology which considers the transfer of ML models from devices with high quality labeled data (called sources) to devices with low quality or unlabeled data (called targets). Our methodology, Source-Target Determination and Link Formation (ST-LF), optimizes both (i) classification of devices into sources and targets and (ii) source-target link formation, in a manner that considers the trade-off between ML model accuracy and communication energy efficiency. To obtain a concrete objective function, we derive a measurable generalization error bound that accounts for estimates of source-target hypothesis deviations and divergences between data distributions. The resulting optimization problem is a mixed-integer signomial program, a class of NP-hard problems, for which we develop an algorithm based on successive convex approximations to solve it tractably. Subsequent numerical evaluations of ST-LF demonstrate that it improves classification accuracy and energy efficiency over state-of-the-art baselines.

==> algos/communication.tex <==
\subsection{Communication Energy Determination}
\label{app_ssec:comm_energy}
Recall the definition of communication energy consumption: $E_{i,j}(\alpha_{i,j}) = K_{i,j}\frac{\alpha_{i,j}}{\alpha_{i,j}+\epsilon_E}$, $\forall i,j \in \mathcal{N}$. 
We here define our method to find $K_{i,j}$ for every $(i,j)$-pair. 
For any given device pair $(i,j)$, we determine $K_{i,j}= \frac{M}{R_{i,j}}P_i$, where $P_i$ is transmission power at device $i$ (watts), $R_{i,j}$ is transmission rate from device $i$ to device $j$ (bits/sec), and $M$ is the size of the hypothesis transmitted in bits. 
For all devices $i \in \mathcal{N}$, we determine the transmission power $P_i$ randomly between $P_{min} = 23 dBm$ and $P_{max} = 25 dBm$. %\footnote{See "Mobile unmanned aerial vehicles (UAVs) for energy-efficient Internet of Things communications" by Mohammad Mozaffari, Walid Saad, Mehdi Bennis, and Merouane Debbah, in \textit{IEEE Transactions on Wireless Communications}, 2017.}. 
Similarly, for all device pairs $(i,j)$, we determine the transmission rate $R_{i,j}$ randomly between $R_{min} = 63$Mbps and $R_{max} = 85$Mbps. 
The size of the hypothesis in bits is assumed to be fixed at $1$Gbit.
{\color{red} In particular, these measurements are similar to commonly used measurements in autonomous systems research~\cite{mozaffari2017mobile}, and their selection was a conscious decision to highlight the versatility of our formulation and optimization methodologies.}


==> algos/optim_pseudocode.tex <==
% \subsection{Pseudocode}
% \label{app_ssec:pseudocode}
% We present the iterative optimization method for $(\boldsymbol{\mathcal{P}})$ in Algorithm~\ref{app_alg:optimization_iteration}. 

% \begin{algorithm}[t] 
%  	\caption{Optimization solver for problem~$\bm{\mathcal{P}}$}\label{alg:cent}
%  	\label{app_alg:optimization_iteration}
%  	\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
%  	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%   	{\footnotesize
%  	\Input{Convergence criterion.}
%  	\Output{$\bm{x}^\star\{\textrm{Objective of $\bm{\mathcal{P}}$ evaluated at $\bm{x}^\star$}\}$}
%  	 }
%  	 Set the iteration count $\ell=0$.\\
%  	 Choose a feasible point $\bm{x}^{[0]}$.\\
%  	 Obtain the monomial approximations~\eqref{app_eq:approx_term_a},\eqref{app_eq:approx_term_b1},\eqref{app_eq:approx_term_b2},\eqref{app_eq:approx_term_c},\eqref{app_eq:posy_con_pos},\eqref{app_eq:posy_con_neg} given $\bm{x}^{[\ell]}$.\label{midAlg1}\\
%  	 Replace the results in the approximation of Problem~$\bm{\mathcal{P}}$ (i.e., $\bm{\mathcal{P}'}$ given by~\eqref{app_eq:prob_prime}-\eqref{app_eq:prob_prime_lasteq} in Appendix~\ref{app_sssec:tx_2gp}).\\
%  	 With logarithmic change of variables, transform the resulting GP problem to a convex problem (as described in Appendix~\ref{app_sssec:gp}).\\
%  	 $\ell=\ell+1$\\
%  	 Obtain the solution of the convex problem using current art solvers (e.g., CVXPY~\cite{diamond2016cvxpy}) to determine  $\bm{x}^{[\ell]}$.\label{Alg:Gpconvexste}\\
%  	 %$\norm{\bm{x}^{[m]}-\bm{x}^{[m-1]}}> \sigma$ 
%  	 \If{two consecutive solutions $\bm{x}^{[\ell-1]}$ and $\bm{x}^{[\ell]}$ do not meet the specified convergence criterion}{
%  	\textrm{Go to line~\ref{midAlg1} and redo the steps using $\bm{x}^{[\ell]}$.}\\\Else{Set the solution of the iterations as $\bm{x}^{\star}=\bm{x}^{[\ell]}$.\label{Alg:point2}\\
%  	}}
% \end{algorithm}



==> borrowed/AG_mean.tex <==
\subsection{Arithmetic-Geometric Mean Inequality}
\label{app_ssec:ag_mean_inequality}

% ~\cite{duffin1972reversed}
\begin{lemma}[\textbf{Arithmetic-geometric mean inequality}\footnote{See "Reversed geometric programs treated by harmonic means" By Richard James Duffin and Elmor L Peterson in \textit{Indiana University Mathematics Journal}, 1972.}]
\label{Lemma:AG_mean}
Consider a posynomial function $g(\bm{y})=\sum_{i=1}^{i'} u_i(\bm{y})$, where $u_i(\bm{y})$ is a monomial, $\forall i$. The following inequality holds:
\begin{equation}\label{eq:approxPosMonMain}
    g(\bm{y})\geq \widehat{g}(\bm{y})\triangleq \prod_{i=1}^{i'} \left( \frac{u_i(\bm{y})}{\alpha_i(\bm{z})} \right)^{\alpha_i(\bm{z})},
\end{equation}
where $\alpha_i(\bm{z})=u_i(\bm{z})/g(\bm{z})$, $\forall i$, and $\bm{z}>0$ is a fixed point.
\end{lemma}



==> sims/gp_conv.tex <==

\subsection{Optimizer Convergence and Source Error Sensitivity}
\label{app_ssec:gp_conv}
In Figs.~\ref{fig:obj_fxn_convergence}-\ref{fig:st_determination_source_error}, we investigate the effect of having a large empirical error on the convergence of Algorithm~\ref{app_alg:optimization_iteration}. We assume here that (i) five devices have labeled or partially labeled datasets and (ii) the other five devices only have unlabeled data. Figs.~\ref{fig:obj_fxn_convergence} indicates that for both settings of empirical error on a labeled dataset, our formulation $(\widehat{\boldsymbol{\mathcal{P}}})$ converges after 20-30 approximation iterations. Fig.~\ref{fig:st_determination_source_error} shows that the large empirical error at device 3 results in $(\widehat{\boldsymbol{\mathcal{P}}})$ classifying that device as a target even though it may have labeled data. 
This means that our methodology is able to determine when a device, may have locally labeled data, but would be better suited as a target device. 

% \begin{figure}[t]
% \centering
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{results/init_test_obj.pdf}
%   \vspace{-1mm}
%   \caption{Convergence of our iterative solver for $(\boldsymbol{\mathcal{P}})$.} 
%   \label{fig:obj_fxn_convergence}
% \end{subfigure}
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{results/init_test_psi.pdf}
%     \vspace{-1mm}
%   \caption{Source/target classification $\psi_i$ at convergence.}
%   \label{fig:st_determination_source_error}
% \end{subfigure}
% \vspace{-1.5mm}
% \caption{Depiction of convergence behavior for Algorithm~\ref{app_alg:optimization_iteration} for two different settings of source errors across devices with labeled/partially labeled data.}
% \end{figure}




% \begin{figure}[t]
% \centering
%   \centering
%   \includegraphics[width=.48\linewidth]{results/init_test_obj.pdf}
%   \vspace{-1mm}
%   \caption{Each device has a mixed dataset.}
%   \label{fig:obj_conv}
% \end{figure}

% \begin{figure}[t]
% \centering
%   \centering
%   \includegraphics[width=.48\linewidth]{results/init_test_psi.pdf}
%   \vspace{-1mm}
%   \caption{Source Error Response.}
%   \label{fig:psi_conv}
% \end{figure}

==> sims/nrg_ratios.tex <==
\subsection{Energy-Dependent Model Ratios Breakdown}
\label{app_ssec:ratios}
In Fig.~\ref{fig:nrg_ratios_phi_e}, we investigate the effect of the energy importance weight $\phi^{\mathsf{E}}$ on the distribution of link formation weights $\boldsymbol{\alpha}$ across target devices in the optimization result. The three columns shown correspond to the columns in Fig.~\ref{fig:phi_e_vary} (i.e., for different datasets), with specific values of $\phi^{\mathsf{E}}$. As $\phi^{\mathsf{E}}$ increases, we see fewer sources communicating with the set of targets in each case. As a result, the link weights for model transfer become skewed to favor only a few sources.

% \begin{figure*}[t]
% \centering
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{results/nrg_model_ratiosM.pdf}
%     \vspace{-1mm}
%   \caption{MNIST}
%   \label{fig:nrg_alpha_M}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{results/nrg_model_ratiosU.pdf}
%     \vspace{-1mm}
%   \caption{USPS}
%   \label{fig:nrg_alpha_U}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{results/nrg_model_ratiosMM.pdf}
%     \vspace{-1mm}
%   \caption{MNIST-M}
%   \label{fig:nrg_alpha_MM}
% \end{subfigure}
% \vspace{-1.5mm}
% \caption{Effect of $\phi^{\mathsf{E}}$ on the link formation weights $\boldsymbol{\alpha}$ for each of the datasets, with the setup corresponding to Fig.~\ref{fig:phi_e_vary}. Similarly to the effects oberved in Fig.~\ref{fig:phi_e_vary}, as $\phi^{\mathsf{E}}$ increases, the number of unique sources that communicate model gradually decreases for all datasets. }
% \label{fig:nrg_ratios_phi_e}
% \vspace{-3mm}
% \end{figure*}


